Membership Testing in Markov Equivalence Classes via Independence Query Oracles

Understanding causal relationships between variables is a fundamental problem with broad impact in numerous scientific fields. While extensive research has been dedicated to learning causal graphs from data, its complementary concept of testing causal relationships has remained largely unexplored. While learning involves the task of recovering the Markov equivalence class (MEC) of the underlying causal graph from observational data, the testing counterpart addresses the following critical question: Given a specific MEC and observational data from some causal graph, can we determine if the data-generating causal graph belongs to the given MEC? We explore constraint-based testing methods by establishing bounds on the required number of conditional independence tests. Our bounds are in terms of the size of the maximum undirected clique ($s$) of the given MEC. In the worst case, we show a lower bound of $\exp(\Omega(s))$ independence tests. We then give an algorithm that resolves the task with $\exp(O(s))$ tests, matching our lower bound. Compared to the learning problem, where algorithms often use a number of independence tests that is exponential in the maximum in-degree, this shows that testing is relatively easier. In particular, it requires exponentially less independence tests in graphs featuring high in-degrees and small clique sizes. Additionally, using the DAG associahedron, we provide a geometric interpretation of testing versus learning and discuss how our testing result can aid learning.

==> content/easytestables.tex <==
\section{Easily testable scenarios}
\begin{center}
\begin{tabular}{||c | c | c | c||} 
 \hline
 Condition & $[\cG]$ ($\cG$ is hidden) & $[\cG']$ ($\cG'$ is given) & Easy or Hard \\ [0.5ex] 
 \hline\hline
 1 & $i-j$ & $i \to j$ or $i \gets j$ & Easy? \\ 
 \hline
  2 & $i \to j$ or $i \gets j$ or $i-j$ & Missing & \Cref{lemma:condition-two}\\
 \hline
 3 & Missing & $i \to j$ or $i \gets j$ & Easy? \\
 \hline
 4 & $i \to j$ & $i \gets j$ & Easy? \\ [1ex] 
    \hline
 5 & Missing & $i-j$ & Hard \\
 \hline
  6 & $i \to j$ or $i \gets j$& $i-j$ &  Hard? \\
 \hline
\end{tabular}
\end{center}
\kk{The last condition should be hard because of the following: Consider the clique example, removing an edge $e$ (except the edge that connects the final two vertices in the clique) from $\cG'$, we end up creating new v-structures and some of the edges in the new graph which were originally un directed in $[\cG']$  will now be directed in $[\cG]$.}


\paragraph{Notation} For any MEC $[\cG](V,E,A)$, we let $V$ denote the set of vertices, $E$ denote the set of edges (oriented and unoriented), and $A$ denote the set of all oriented edges.

\begin{lemma}[Condition 1]
    \kk{I don't yet have a proof for this lemma}
    Let $[\cG'](V',E',A')$ and $[\cG](V,E,A)$ be the MEC corresponding to given DAG $\cG'$ and the hidden DAG $\cG$. Let $i,j \in V$ be such that $(i,j) \not \in A$ and $(i,j) \in A'$, then in polynomial number of independence tests we can test whether $[\cG']=[\cG]$ or $[\cG'] \neq [\cG]$.
\end{lemma}
\begin{proof}
    Without loss of generality let the orientation of the edge $(i,j)$ be $i \to j$ in $[\cG']$. 
    
    \paragraph{Case 1}: $i \to j$ is part of a v-structure. Let $i \to j \gets k$ be this v-structure, which implies that $i$ and $k$ are not connected in $\cG'$. 
\end{proof}


\begin{lemma}[Condition 2]\label{lemma:condition-two}
    Let $[\cG'](V',E',A')$ and $[\cG](V,E,A)$ be the MEC corresponding to given DAG $\cG'$ and the hidden DAG $\cG$. Let $i,j \in V$ be such that $(i,j) \in E$ and $(i,j) \not \in E'$, then in polynomial number of independence tests we can test whether $[\cG']=[\cG]$ or $[\cG'] \neq [\cG]$.
\end{lemma}
\begin{proof}
    Given $\cG'$ and an vertices $i,j$ such that $(i,j) \not \in E'$, it is immediate to find a set $S$ ($S=\pa(i)$ or $S=\pa(j)$) such that $i \ci j|S$. However as $(i,j) \in E$, we have that $i \nci j|S$ in $\cG$. Therefore it is easy to test whether $[\cG']=[\cG]$ or $[\cG'] \neq [\cG]$ and we conclude the proof.
\end{proof}

\begin{lemma}[Condition 3]
    
\end{lemma}

\begin{lemma}[Condition 4]
    
\end{lemma}



